Unsupervised Discovery of Semantic Latent Directions in Diffusion Models

Despite the success of diffusion models (DMs), we still lack a thorough understanding of their latent space. While image editing with GANs builds upon latent space, DMs rely on editing the conditions such as text prompts. We present an unsupervised method to discover interpretable editing directions for the latent variables $\mathbf{x}_t \in \mathcal{X}$ of DMs. Our method adopts Riemannian geometry between $\mathcal{X}$ and the intermediate feature maps $\mathcal{H}$ of the U-Nets to provide a deep understanding over the geometrical structure of $\mathcal{X}$. The discovered semantic latent directions mostly yield disentangled attribute changes, and they are globally consistent across different samples. Furthermore, editing in earlier timesteps edits coarse attributes, while ones in later timesteps focus on high-frequency details. We define the curvedness of a line segment between samples to show that $\mathcal{X}$ is a curved manifold. Experiments on different baselines and datasets demonstrate the effectiveness of our method even on Stable Diffusion. Our source code will be publicly available for the future researchers.

==> experiment_bin.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{figure/local_celeba.pdf}
    \caption{\textbf{Bold thing.} results of local basis }
    \label{fig:local_basis}
\end{figure}


\section{Experiments}

We validate our methods through a series of empirical experiments and conducted a comprehensive analysis of the latent space of Diffusion Models (DMs). In Section 4.1, we have demonstrated the results of sample editing utilizing the local and global direction found using our proposed methods. In Section 4.2, we have carried out a more in-depth analysis of the latent space of DMs from a geometric perspective. In Section 4.3, we have shown that our methods also work in stable-diffusion. Finally, in Section 4.4, we have verified our proposed methods through an ablation study.

Note that all models employed in this study are official pretrained checkpoints, and their parameters were kept frozen during the experimentation. The implementation details of our method are provided in the appendix. The source code for our experiments is included in the supplementary materials, and will be made publicly available upon publication.



% In this section, we present the results of our experiments using the local basis method and provide an analysis of them. Based on this analysis, we propose an  insight into the generation process of diffusion models at different time steps, as well as a method for obtaining the global basis. Our findings also explain a new interpretation of the interpolation process in diffusion models.

\subsection{Editing Image with Discovered Direction}

%In this subsection, we show the effectiveness of semantic editing with our discovered meaningful directions. We implement our method on CelebA-HQ with DDPM and AFHQ-dog with iDDPM. 
%Please note that all models are official pretrained checkpoints and are kept frozen. Implementation details are described in Appendix. The code is attached to the supplementary materials andwill be available online with publication.

%In this subsection, we demonstrate the effectiveness of semantic editing utilizing the meaningful directions discovered by our proposed method. We conduct our experiments on the CelebA-HQ dataset \cite{karras2018progressive} with the DDPM model \cite{ho2020denoising}, as well as the AFHQ-dog dataset \cite{choi2018stargan} with the iDDPM model \cite{nichol2021improved}. 


% \subsection{local direction}
\label{sec:local}


\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{figure/local_afhq.pdf}
    \caption{\textbf{Bold thing.} results of local basis AFHQ }
    \label{fig:local_basis_afhq}
\end{figure}

% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=0.8\linewidth]{example-image-duck}
%     \caption{\textbf{Bold thing.} results of local basis AFHQ }
%     \label{fig:local_basis_afhq}
% \end{figure}

\paragraph{local}
In \sref{sec:method_local}, our proposed method enables the extraction of multiple semantic editing directions from the local basis for each image. To demonstrate the effectiveness of our approach, we conduct experiments on the CelebA-HQ dataset \cite{karras2018progressive} with the DDPM model \cite{ho2020denoising}, as well as the AFHQ-dog dataset \cite{choi2018stargan} with the iDDPM model \cite{nichol2021improved}.
As depicted in Figure \ref{fig:local_basis}, the local basis obtained via our method can yield highly impactful results in image editing. At time step $t=0.5T$, we are able to identify editing directions that pertain to small adjustments in make-up, facial expression, hair texture, and wrinkles, while at $t=T$, more substantial editing directions such as changes in overall hair color or the addition or removal of hair become discernible. This trend is also evident in the results obtained from the AFHQ-dog dataset, as shown in \fref{fig:local_basis_afhq}.
This provides strong validation for the effectiveness of our geometric approach in semantic image editing.


%At time step $t=0.5T$, we are able to identify editing directions that pertain to small adjustments such as make-up, facial expression, hair texture, and wrinkles, while at $t=T$, more substantial editing directions such as changes in overall hair color or the addition or removal of hair become discernible. 

%In section 3.2, our approach allows for the extraction of $n$ directions from the local basis for each image. As shown in \fref{fig:local_basis}, the local basis obtained can produce significant results in image editing.  % geometrical assumption
%\mingi{At time $t=0.5T$, we can identify editing directions pertaining to adjustments in make-up, facial expression (e.g. smiling), hair texture, and wrinkles. As time progresses to $t=T$, more significant editing directions such as changes in overall hair color or the addition or removal of hair become evident. \fref{fig:local_basis_afhq} shows similar tendency in AFHQ.
%This confirms the validity of our geometrical \yh{approach}. Furthermore, we suppose that it posits a correlation between the editing direction and the corresponding time step, $t$, which will be explored in greater detail in \ref{sec:timestep}. We provide consecutive editing results in \aref{}.} 

\yh{
%Furthermore, we observed a relationship between the fine-to-coarse feature of editing direction with time step $t$. For example, at $t = 0.5T$, editing directions corresponding to make-up, smiling, hair texture, and wrinkles can be found. On the other hand, in case where $t = 1T$, the direction such as changes in the color of the entire hair or the addition or removal of hair, can be found. This implies that the meaningful directions discovered by our method exhibit a coarse-to-fine dependency on time step $t$. A quantitative analysis of this phenomenon will be conducted in a \sref{sec:timestep}.
}

%Furthermore, we posit that there exists a correlation between the editing direction and the corresponding time step in the generative process. The coarse-to-fine generation of DMs has been previously demonstrated in \cite{kwon2022diffusion,choi2022perception} by the results of the diffusion process, however, our approach allows for more direct visualization and analysis of this phenomenon. As the discovered editing directions represent the greatest variations in the \ehspace{}, they can be interpreted as the features that the model is focusing on at each time step.


% We also provide an analysis of semantic editing based on our experimental results and the time step. Previous studies have established that the concentration of the diffusion model varies with t, with the model producing a coarse-to-fine progression as t decreases from T to 0. However, prior literature has not provided a direct analysis of this phenomenon.

% As seen in Figure 4, our results indicate that as t increases from 0.5T, the edits become increasingly coarse. For example, at t = 0.5T, editing directions corresponding to make-up, smiling, hair texture, and wrinkles can be found. Conversely, as t gets closer to T, the direction of coarse changes, such as changes in the color of the entire hair or the addition or removal of hair, can be found

%%% indepth section 에서 쓰기 %%%
% We also provide an analysis of semantic editing based on our experimental results and the time step. Previous studies have established that the concentration of the diffusion model varies with $t$, with the model producing a coarse-to-fine progression as t decreases from $T$ to $0$. However, prior literature has not provided a direct analysis of this phenomenon. \cite{kwon2022diffusion,choi2022perception, daras2022multiresolution}

% 용현쓰
%1. local basis 에서 보면 t/T = 1 일수록 coarse 한 변화가 일어나고, t/T ~ 0 이면 fine 한 변화가 발생하는걸 관찰했다. 진짜 그럴까?2. PSD 확인해보니 진짜 그랬다. 이는 모델이 주목하는 정보의 frequency 가 t 에 의해 조절됨을 의미한다. 

% In this paper, we aim to analyze which attributes are considered coarse and which are considered fine in the diffusion model.

%The concepts of "coarse" and "fine" can be abstract and open to interpretation. Generally, overall form is considered coarse, while facial changes such as smiling are considered fine. However, determining which edits are considered coarse or fine can be subjective. For example, is changing hair color a more coarse edit than changing race? Our analysis, as shown in \fref{fig:local_basis}, suggests that changing hair color is more coarse. We suppose that the degree of color change in a wide area is the criterion for defining coarse and fine edits in the diffusion model.

% As seen in \fref{fig:local_basis}, our results indicate that as $t$ increases from $0.5T$, the edits become increasingly coarse. For example, at $t = 0.5T$, editing directions corresponding to make-up, smiling, hair texture, and wrinkles can be found. Conversely, as t gets closer to T, the direction of coarse changes, such as changes in the color of the entire hair or the addition or removal of hair, can be found. 
%However, it is important to note that these distinctions between coarse and fine edits are determined based on the characteristics of the diffusion model, and may differ from subjective interpretations of what constitutes coarse or fine changes. 

%Additionally, we also noticed that at this stage, the direction of long hair becomes entangled with the woman attribute, highlighting the complexity of disentangling semantics.

%We observed that the local basis generates distinct editing results at different timesteps. Previous studies have suggested that the DMs can produce varying outputs depending on t \cite{kwon2022diffusion,choi2022perception}, however, they did not provide an analysis of how or what attributes the model focuses on.  

%In our experiments, we have observed that the local basis generates distinct editing results at different timesteps, providing evidence of the varying semantics that can be altered as a function of t. Our findings suggest that this variation in semantics is closely related to the changes in color that the semantic editing will bring. Through a thorough analysis of \fref{fig:local_basis}, we have identified that at $t = 0.5T$, we are able to find directions that modify existing colors, such as makeup and hair texture, or change parts of the face, such as smiling and wrinkles, providing a high level of granularity in semantic editing. As $t$ increases to 0.75, the range of change becomes wider, allowing for the identification of directions that change the entire color of the face, or add colors that were not originally present, such as a beard, as well as wide-area changes, such as becoming an Asian or a woman. At $t = T$, we were able to identify directions that change the entire color of the hair, and directions that add or remove hair. This level of control allows for a wide range of semantic editing options. However, we also noticed that at this stage, the direction of long hair becomes entangled with the woman attribute, highlighting the complexity of disentangling semantics.

% For example, a beard that seems to be an intuitive fine area should change the color of the area around the chin a lot from a color perspective. On the other hand, gender changes, which seem to be intuitively coarse areas, should be changed overall, but the change in pixel units is not very large. As a result, the editing direction corresponding to the beard and gender can be found in the same time step. This demonstrates the importance of considering both the range of changes and the specific attributes being edited when interpreting the results obtained from the diffusion model.

%Our experiments using the local basis method have shown that it is capable of significant image editing, as demonstrated in Figure 3. The horizontal axis represents the change in each direction, and examples of editing such as rotation, gender transformation, and makeup application can be seen. This result allows us to conclude the following:

%\paragraph{Model Focus Evolution over $t$} Our experiments have shown that the local basis method allows for significant image editing, as demonstrated in Figure 4. The vertical axis represents the time steps, and it is clear that the basis tends to change according to the direction found for each time step. Large changes are observed when t is large, and small changes when t is small. This can also be seen through the visualization of dx in Figure 4b, where it can be seen that the direction obtained from the same image has a higher frequency as t decreases. This demonstrates the evolution of the model's focus on features at different time steps.

\paragraph{t}
Furthermore, we posit that there exists a correlation between the editing direction and the corresponding time step in the generative process. The coarse-to-fine generation of DMs has been previously demonstrated in (Kwon), however, our approach allows for a more direct visualization of this phenomenon. As the discovered editing directions represent the greatest variations in the h-space, they can be interpreted as the features that the model is focusing on at each time step.
By analyzing the visual representation of vk in Figure (a), we argue that the model initially focuses on coarse information at the beginning of the generative process and then gradually shifts its attention to finer details as time progresses.
To further support this observation, we calculate the power spectral density (PSD) based on the frequency of $\dx{}$ obtained at each timestep. Figure \ref{fig:PSD} (b) illustrates that as $t$ approaches T, the PSD contains a higher proportion of low-frequency information, whereas as $t$ approaches 0, it contains a higher proportion of high-frequency information. This supports our argument that the model's focus shifts from coarse to fine details as the generative process progresses.

\paragraph{global}
As previously established in Section 3, the properties of the editing directions are particularly homogeneous when $t \approx T$. This implies that the features that the model focuses on at the end of the generative process are similar across different samples. To exploit this observation, we propose a method for obtaining a global basis by averaging similar editing directions. Our approach involves sampling latent variables $\mathbf{x}_T \sim \mathcal{N}(0, I)$ and then collecting similar directions from each $\mathbf{x}_T$'s local basis.
The results of the editing based on the global directions can be found in Figures \ref{fig:global_basis} and \ref{fig:global_basis_afhq}, which demonstrate that similar directions have a consistent impact on semantic editing across different samples. Additional results can be found in the appendix \aref{}.

% 

% \subsubsection{Global Direction}
% \label{sec:global}
% 원래 있던것
%In section \sref{sec:method_global}, we have established that we can identify good pairs of directions in two different local bases, as illustrated in \fref{fig:homogenity}. Thus, we proposed a method for obtaining the global basis by averaging similar directions. To discover the global directions, we first sample latent variables $\mathbf{x}_T \sim \mathcal{N}(0, I)$ and then collected the similar directions from each $\mathbf{x}_T$'s local basis. The editing results based on global direction can be found in \fref{fig:global_basis}, \ref{fig:global_basis_afhq} which shows the same directions affect the same semantic editing. We provide additional results in \aref{}.
%, including blonde hair, dark skin, \todo{appendix figure 나오면 채우기}, can be found


% 하지만, 그에 반해 t 가 T 에서 멀어질수록, sample 간 consistency 가 줄어들었다. This may be attributed to the fact that the manifold hypothesis may not work when denoising process is processed. \cite{zhang2022gddim} 또한, local basis 끼리의 homogenity 가 줄어들어서 그런 것도 있다. 굵직한 feature 는 그 종류가 한정적인 것에 반해 fine 한 feature 일수록 sample 별로 다양한 조작이 가능한것을 생각할 수 있다. 이는 eigenvalue spectrum 이 t ~ 0 로 갈수록 완만해지는 것으로부터 양적으로도 확인할 수 있다. (Appendix figure)

% Our experiments revealed that some directions in the local basis had a similar cosine similarity, as illustrated in \fref{fig:homogenity}. Therefore, we proposed a method for obtaining the global basis by averaging the similar $\dx{}$. The resulting global direction showed better performance when $t = T$, however, its effectiveness was limited when $t$ did not equal $T$. This may be attributed to the fact that the manifold of $\mathbf{x}_t$ may not be a perfect Riemannian manifold when $t$ is too small compared to $T$.

% Despite these limitations, the global direction found at $T$ yielded interesting results. As shown in \fref{fig:global_basis}, by using the average of similar local directions obtained from 100 random noise as the global direction, we were able to find rotation directions in addition to the generally conceivable young direction.

%This is particularly noteworthy as rotation direction is an editing direction that can be easily found in GANs, however, it has not been observed in Diffusion models which are known to maintain the spatial information of the input.

% In conclusion, our experiments demonstrate the feasibility of obtaining global basis through averaging similar local directions. The global direction found at $T$ showed promising results, including the discovery of a previously unseen rotation direction.

\begin{figure}[!t]
    \centering
    \includegraphics[width=1.0\linewidth]{figure/global_celeba.pdf}
    \caption{\textbf{Bold thing.} results of global basis }
    \label{fig:global_basis}
\end{figure}




\subsection{Indepth Analysis on the latent space of DMs} 
%In this chapter, we investigate the properties of diffusion models (DM) using geometric methods. We begin by analyzing the frequency domain of the discovered meaningful direction, which allows us to reveal that the frequency domain of meaningful features that the DM is focusing on is controlled by the time parameter $t$. Additionally, we analyze the global geometric structure of the \exspace{}. Specifically, we demonstrate that the \exspace{} is a spherically warped space by showing that x-space slerp is close to the geodesic. This improves our understanding of the spatial structure of the DM in the x-space and provides a geometric understanding of why slerp is a superior interpolation scheme for latent variables in DM.

\begin{figure}[!t]
    \centering
    \includegraphics[width=1.0\linewidth]{figure/afhq_global.pdf}
    \caption{\textbf{Bold thing.} results of global basis }
    \label{fig:global_basis_afhq}
% \end{figure}

% \begin{figure}[!t]
%     \centering
    \includegraphics[width=1\linewidth]{figure/freq.pdf}
    \caption{
        The analysis of the effect of $t$ on $\mathbf{v}_k$. (a) the sample editing trajectory and the visualization of $\mathbf{v}_k$. Since the size of $\mathbf{v}_k$ is very small, normalization was applied for better visualization. 
        % The sample editing trajectory illustrates that as t decreases, editing occurs at finer region. (e.g. hair texture) The visualization of $\mathbf{v}_k$ suggests that these changes correspond to fine features as t decreases. 
        (b) the Power Spectral Density (PSD) of $\mathbf{v}_k$. The PSD at 1T (blue line) shows that it is the time step which has strongest low-frequency signals during denoising process. On the other hand, as $t$ decreases, a large number of (red) high frequency signals are contained.
        On the other hand, as $t$ decreases, high frequency information contained in $\mathbf{v}_k$ increases.
    }
    \label{fig:PSD}
\end{figure}


\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.8\linewidth]{./figure/slerp_lerp.pdf}
    \caption{
    Inspect the warpage of $\mathcal{X}$. 
    (a) Conceptual illustration of our result. Our experiments demonstrate that x-space lerp represents a curved path that deviates in h-space, while x-space slerp follows a relatively parallel path, providing a better trajectory.
    (b) Geodesic metric. We measure the local warpage of the space at each step of the trajectory. The shaded region represents the mean $\pm$ 0.5 sigma. Note that the geodesic in this case is obtained not by interpolation between two points, but by geodesic shooting.
    \todo{그래프 geodesic 에 approx 라고 작성해두기}}
    \label{fig:slerp_lerp}
\end{figure*}

%In this chapter, we delve deeper into the properties of diffusion models (DM) by utilizing geometric methods. We begin by examining the frequency domain of the discovered meaningful direction. This allows us to reveal that the frequency domain of meaningful features that the DM is focusing on is controlled by the time parameter $t$. Additionally, we analyze the global geometric structure of the $\mathcal{X}$. Specifically, we demonstrate that the $\mathcal{X}$ is spherically warped space, by showing that \exspace{} slerp is close to the geodesic. This improves our understanding of the geometrical structure of the latent space of the DM and provides a geometric understanding of why slerp is a superior interpolation scheme for latent variables in DM.  

% 1. 이번 챕터에서는 지금까지 활용한 기하적인 방법을 활용해서 DM 의 성질을 더욱 깊게 분석한다. 2. 먼저, x space local basis 의 power spectral density 를 봄으로써 모델이 주목하는 feature 의 frequency domain 이 t 에 의해 조절됨을 밝혔다. 이는 DM 의 생성 메커니즘에 대한 이해를 높여준다. 3. 이후, h space 와 x space 의 global 한 기하적 구조를 분석한다. 특히, 우리는 x space slerp 이 h space geodesic 에 가까움을 밝혔다. 이는 DM 의 x space 와 h space 의 공간 구조에 대한 이해를 키워준다.




% \subsubsection{$t$ controls which frequency the model will focus on}
% \label{sec:timestep}
% In the previous section, we discovered that as the value of time step $t$ decreases, editing becomes increasingly fine, and conversely, as the value of time step $t$ increases, editing becomes increasingly coarse. As our discovered direction represents the greatest variation in the h-space, it can be interpreted as the feature that the model is focusing on. Based on these observations, we hypothesized: Does the model focus on coarse information at the beginning of the denoising process and then on detailed feature as the denoising process?

% To support this observation, the power spectral density (PSD) was calculated based on the frequency of $\dx{}$ obtained at each timestep. Figure \ref{fig:PSD} illustrates that as $t$ approaches T, the PSD contains a higher proportion of low frequency information, whereas as $t$ approaches 0, it contains a higher proportion of high frequency information. This is also supported by the visualization of $\dx{}$ in Figure \ref{fig:PSD}. 

% {\color{gray} In addition, we revealed that this phenomenon is not caused by the latent variable, but by the time parameter $t$. This can be verified by looking at the PSD changing the time parameter $t$ while the sample x is fixed. As shown in figure, it can be seen that the information the model pays attention to is transferred to high frequency as $t$ approaches to 0, even though the image has not been changed at all.}

% % 우리 실험 결과에 의미 부여하기.
% Previous studies have established that the concentration of the diffusion model varies with $t$, with the model producing a coarse-to-fine progression as t decreases from $T$ to $0$. However, prior literature has not provided a direct analysis of this phenomenon. \cite{kwon2022diffusion,choi2022perception, daras2022multiresolution} Our observation explains the well-known phenomenon that the DM initially generate on relatively coarse features, and subsequently generate on fine features in the latter stages. 

% In fact, these categories of coars and fine can be classified in terms of frequency. To support this observation, we calculated the power spectral density (PSD) according to the frequency of $\dx{}$ obtained at each timestep. \fref{fig:PSD} illustrates that as $t$ approaches T, the PSD contains more low frequency information and as $t$ approaches 0, it contains more high frequency information. This is also supported by the visualization of $\dx{}$ in \fref{fig:PSD} (a). Through this analysis, we can gain a deeper understanding of which features the DMs pay attention to according to local basis.


% \subsubsection{Global Warpage of \exspace{}}

In Section 3, we propose a method for parallel transport in the h-space, under the assumption that the x-space is not a semantically flat manifold. This section provides evidence that the x-space is in fact a curved manifold and offers insights into the global geometrical structure of the x-space through local information. However, it can be difficult to directly infer the curvature of the x-space. To address this challenge, we propose an analysis of the trajectory between two points in x-space. Specifically, we use the Lerp trajectory, which is indicative of a flat manifold, and the Slerp trajectory, which is indicative of a curved manifold. By comparing the degree of separation between the local tangent spaces of each trajectory, we can provide a quantitative measure of the degree to which the x-space is curved.



% Thus far, we focus only on the local geometric properties of the \exspace{}. Then our next question is "Can we gain insight into the global geometrical structure of $\mathcal{X}$?" Since we only have access to local geometric information, we must infer the global structure by combining local information. This can be achieved by following curves and investigate the global structure through an examination of local warpage. Through this method, we have demonstrated that the x-space is spherically warped space.

% 1. 지금까지 우리는 x space 의 local 한 기하적 대상에 대해 다뤄왔다. 그렇다면 x space 의 global 한 공간적 특성을 알 수 없을까? 앞선 section 과 마찬가지로 x space 의 공간을 h space 에 의존해서 분석할 수 있다. 우리는 x 위의 curve 따라가면서 local 한 휘어짐을 조사하는 방식으로 global 구조를 간접적으로 조사했다. 우리는 이를 통해 x space 의 slerp 이 lerp 에 비해 h space 에서 덜 휘어진 경로임을 보였다.


In order to investigate how curved the space is, we have to define a metric to measure the warpage. In our work, we used \emph{Geodesic metric}. \cite{choi2021not, ye2016schubert} Conceptually, the Geodesic metric can be understood as a measure of the angle between two different vector spaces. Thus, the geodesic metric of two tangent spaces gives us information about how much space bends between two points. 
Given two tangent space $\mathcal{T}_{\mathbf{x}_i}, \mathcal{T}_{\mathbf{x}_j}$, the Geodesic metric is defined as below : 
\begin{equation}
d_{\text{geo}}(\mathcal{T}_{\mathbf{x}_i}, \mathcal{T}_{\mathbf{x}_j}) = \sqrt{\sum_k \theta_k^2}
\end{equation}
where, $\theta_k = \cos^{-1}(\sigma_k(U_i^{\tran}U_j)$ denotes the $k$-th principle angle between $\mathcal{T}_{\mathbf{x}_i}$ and $\mathcal{T}_{\mathbf{x}_j}$. Here, $U_i$ is the column-wise orthonormal matrix of which columns span $\mathcal{T}_{\mathbf{x}_i}$ and $\sigma_k(U_i^{\tran}U_j)$ is $k$-th singular value of $U_i^{\tran}U_j$. 

% \equation{Grassman metric}
% Our experiment proceeds through the following three steps. Firstly, we plot curves (slerp, lerp, geodesic) on the \exspace{}. Here, the geodesic between arbitrary two points is intractable, thus we consider the curve given by geodesic shooting as a geodesic. This curve is not a geodesic between two points, but still can be interpreted as a lower bound on the warpage of a path. Second, we transfer these curves to the $\mathcal{H}$ via $f$. Lastly, following along the curve, measure how much the local warpage of space. This is done by measuring the Geodesic metric between $\mathcal{T}_h$, and $\mathcal{T}_{h'}$, where $h'$ is a next interpolation point. curves that are closer to geodesic will represent an untwisted curve.

Our experiment proceeds through the following three steps. Firstly, we plot curves on the \exspace{}. Second, we transfer these curves to the $\mathcal{H}$ via $f$. Lastly, following along the curve, measure how much the local warpage of space. This is done by measuring the Geodesic metric between $\mathcal{T}_h$, and $\mathcal{T}_{h'}$, where $h'$ is a next interpolation point. 

% 3. 우리의 실험은 다음 3가지 과정을 거친다. 먼저, x space 위에 curve (slerp, lerp, geodesic) 를 그린다. 이후, 이 curve 를 f 를 통해 h space 로 옮긴다. 마지막으로, h space 의 curve 를 따라가면서 공간의 국소적인 휘어짐을 측정한다. 이때, 덜 휘는 curve 일수록 geodesic 에 가깝고, x space 에서 휘어지지 않은 curve 임을 나타낸다. 


For relative comparison, we are showing Slerp, lerp, and geodesic in figures. Here, the geodesic between arbitrary two points is intractable, thus we consider the curve given by geodesic shooting as a geodesic. This curve is not a geodesic between two points, but still can be interpreted as a lower bound on the warpage of a path. curves that are closer to geodesic will represent an untwisted curve. 

From the graph, it can be observed that lerp (the blue line) traverses a drastic curved path at the beginning and end of the curve, which suggests that when lerp moves away from the surface of the Gaussian prior and towards the center, it experiences a sudden change in the curvature of space. On the other hand, slerp and geodesic choose paths that maintain a consistent level of local warping throughout the entire curve, which suggests that slerp in the x-space results in a path that is closer to the geodesic compared to lerp. Lerp의 결과는 x space가 휘어져있다는 것을 암시한다. 더 나아가서 The similarity in behavior between slerp and geodesic suggests that the x-space is a spherically curved space, which explains why slerp interpolation has performed well in xT from a geometric perspective.



%The rightmost figure in \fref{fig:slerp_lerp} illustrates the warping of slerp, lerp, and geodesic. From the graph, it can be observed that lerp (the blue line) traverses a drastic curved path at the beginning and end of the curve, which suggests that when lerp moves away from the surface of the Gaussian prior and towards the center, it experiences a sudden change in the curvature of space. On the other hand, slerp and geodesic choose paths that maintain a consistent level of local warping throughout the entire curve, which suggests that slerp in the x-space results in a path that is closer to the geodesic compared to lerp. The similarity in behavior between slerp and geodesic suggests that the x-space is a spherically curved space, which explains why slerp interpolation has performed well in xT from a geometric perspective.
                    
% 4. \fref{fig:PSD} 의 가장 오른쪽 figure 는 x space 에서의 slerp, lerp 과 geodesic 의 warpage 를 나타낸 것이다. 여기서 임의의 두 점에 대한 geodesic 은 intratable 하기에, geodesic shooting 으로 구한 geodesic 을 사용했다. 이는 임의의 경로를 이동할때 휘어지는 것에 lowerbound 로 해석할 수 있다. 그래프를 살펴보면, 모든 interpolation point 에 대해 blue line (lerp) 이 orange line (slerp) 에 비해 더 휘어진 경로를 이동하는 것을 알 수 있다. 이는 x space 에서의 slerp 이 lerp 에 비해 평행선에 더 가까운 path 임을 알려준다. slerp 이 평행선이라는 것은 x space 가 동그랗게 휘어졌다는 정보를 알려준다. 이는 현재까지 xT 에서 우리가 slerp interpolation 이 잘 작동했었던 기하적인 이유를 설명해준다.





\subsection{Stable Diffusion} % Text-conditional Diffusion model
In this section, we demonstrates versatility of our method by showing its applicability to stable diffusion. We also demonstrate that our method can discover meaningful directions of Latent Diffusion Models (LDMs) to achieve editing. 
%In this experiment, we employed the stable diffusion 1.5v model \cite{rombach2022high}. 
The key difference between LDMs and previous settings is the incorporation of a text conditional component, which allows for the use of a prompt to guide the generation of images. 
%To minimize the effect of classifier-free guidance, the guidance scale was fixed to 1.

The results for editing based on discovered local directions are illustrated in \fref{fig:ldm_local}. As expected, the closer the value of t is to T, the more global changes, such as frame and foggy editing, are observed, while the closer t is to 0, the more texture-based manipulations, such as those of OO and OO, are produced. we could also find that the meaningful directions are influenced by the chosen prompt. For example, the direction of portrait manipulation found in the Vangogh prompt can not be found in local basis given Cyberpunk prompt.

In terms of global results, we could able to find several the meaningful directions. For example, in the Vangogh prompt, we were able to identify directions for frame manipulation, whereas in the Cyberpunk prompt for foggy city manipulation. One limitation of our method on the stable diffusion model is that it sometimes results in unexpected large editing in one step. This phenomenon made it difficult to interpret what each editing direction was about. This phenomenon will be covered in more detail in the limitation section.

\begin{figure}[!t]
    \centering
    \includegraphics[width=1\linewidth]{figure/LDM_local.pdf}
    \caption{\textbf{Bold thing.} LDM local }
    \label{fig:ldm_local}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=1\linewidth]{figure/LDM_global.pdf}
    \caption{\textbf{Bold thing.} LDM global }
    \label{fig:ldm_global}
\end{figure}

% 0. 우리는 stable diffusion 1.5v 을 사용했다. \cite{rombach2022high}
% 1. 먼저 기존 setting 과 stable diffusion 이 다른 부분은 text conditional 부분이다. 우리는 이미지를 잘 설명하는 prompt 를 선택했다.
% 2. 또한, classifier-free guidance 에 의한 효과를 최대한 없애주기 위해 guidance scale 을 1로 고정했다. 이로써, text conditional model 로만 생성하게 된다. 
% 3. local direction 에 대한 결과는 figure 에 나와있다. 먼저, section 3 에서 살펴봤던 t 에 의한 fine-to-coarse 효과는 그대로 나타나는 것을 확인할 수 있었다. t 가 T 에 가까울수록 액자, foggy 등 전체 이미지에 영향을 주는 조작이 이뤄지는 반면, t 가 0 에 가까울수록 카툰이나 OO 등 질감에 대한 조작이 나타난다. stable diffusion 에서 새롭게 살펴볼 수 있는 부분은 prompt 에 의해 meaningful direction 이 달라진다는 점이다. 예를 들어, vangogh 에서 찾아볼 수 있었던 초상화에 대한 방향은 cyberpunk 에서는 찾아보기 어려웠다.
% 2. global 결과 : prompt 에 따라 meaningful direction 이 달라진다. Vangogh 에서는 액자로 가게 하는 방향, Cyberpunk city foggy 방향을 찾을 수 있었다. 하지만, Stable diffusion 은 한번의 step 으로 지나치게 큰 editing 이 발생할 때가 있어서 sample 간 consistency 를 확인하기 어려웠다. 이런 현상이 발생하는 이유는 edit 할때 더해주는 v 의 크기가 $v^\tran v$ 으로 고정되기 때문에 발생한다. 이는 $\mathcal{X}$ 의 metric 이 공간마다 유사하다는 가정을 담고 있다. 
% 하지만, LDM is already a diffusion model on the latent space of VAE 이기 때문에 $\mathcal{Z}$ 에서 edit 이 이뤄지고 있고 $v^\tran v$ 보다 $\mathcal{Z}$ 공간에 더 맞는 metric 에 맞춰서 부여돼야 한다. \cite{arvanitidis2017latent, arvanitidis2020geometrically} Nevertheless, we can find meaningful local, global directions in LDM, indicating that LDM is still a promising research topic for deeper study.


\subsection{Ablation}
In this chapter, we conduct a comprehensive ablation study to evaluate the effectiveness of our proposed method in comparison to alternative approaches. We begin by assessing the impact of incorporating random directions into the latent variable of DMs, as depicted in \fref{fig:ablation_random_dx_ours} (a). The results demonstrate that the inclusion of random directions leads to a significant degradation in image quality, characterized by an excessive level of noise and shape distortion. This highlights the importance of semantics in the latent variable of DMs, and the difficulty of finding meaningful directions in its absence.

\todo{여기 stepsize 에 대한 ablation 이 들어가면 좋을듯. Parallel Transport}

Next, we examine the effect of adding $\dx{}$ directly without utilizing the \iasyrp{} method, as shown in \fref{fig:ablation_direct_dx_ours} (b). The results reveal that this approach also results in a substantial degree of noise in the image, as well as uneven semantic changes. This is due to the lack of calibration to maintain the distribution of $\mathbf{x}_t$, which leads to semantic changes occurring unevenly. As detailed in the appendix, when calibration is performed to preserve the distribution of $\mathbf{x}_t$, the semantic changes are not consistent.

Finally, we present the results of our proposed method, as illustrated in \fref{fig:ablation_random_dx_ours} (c). Our approach utilizes the reverse process by obtaining the $\mathbf{x}_t$t corresponding to editing, allowing for the successful execution of high-quality image editing without the presence of noise or shape distortion. The results demonstrate the superiority of our method in comparison to alternative approaches, and highlights the importance of semantics and calibration in achieving high-quality image editing.

\begin{figure}[!t]
    \centering
    \includegraphics[width=1\linewidth]{figure/random.pdf}
    \caption{Random direction ablation study. If we add a random direction instead of the meaningful direction we have identified, we could only see artifact rather than semantic editing.
}
    \label{fig:ablation_random_dx_ours}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=1\linewidth]{figure/direct.pdf}
    \caption{\textbf{Bold thing.} direct vs ours }
    \label{fig:ablation_direct_dx_ours}
\end{figure}

\subsection{Comparison}
In addition to our proposed method, we also conduct experiments with GANspace as a point of comparison. Our approach involves utilizing GANspace by considering $\mathbf{x}_t$ as the latent variable $\mathbf{z}$ of GANs and \ehspace{} as the \emph{w space} of GANs. The results of this experiment are depicted in \fref{fig:ganspace}, which illustrates the editing results obtained through the direction found in GANspace. As can be seen from the figures, the editing direction found using the GANspace method primarily alters the color of the image. This suggests that simply collecting all $hs$ and finding the principal axes through PCA may result in finding the axes that control the overall color. Additional GANspace results can be found in the appendix.

In contrast, our method is designed to find the direction that can bring about the greatest change in \ehspace{} at each $\mathbf{x}_t$, enabling semantical editing. Thus, this approach is believed to be more effective in achieving semantical editing than the GANspace method.

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.8\linewidth]{figure/GANspace.pdf}
    \caption{\textbf{Bold thing.} GANspace }
    \label{fig:ganspace}
\end{figure}



==> trashbin.tex <==
\section{abstract}

% This paper introduces a new method to control the generative process of Diffusion Models (DMs), which are highly powerful generative models that have shown great performance in various tasks. Our method provides useful intuitions on the latent space of DMs in an unsupervised manner, allowing us to manipulate the resulting images using Riemannian geometry. We first identify directions in the latent space that can be used to manipulate the images, by using the singular value decomposition of the Jacobian of the mapping from the latent space to the intermediate feature space of the model. We then find global directions by exploiting the homogeneity of the intermediate feature space, which removes the need for cumbersome per-sample Jacobian computation and allows for general controllability. Our method also shows interesting properties of DMs such as smooth interpolation between samples by spherical linear interpolation is approximately geodesic in the feature space, and the relationship between timesteps and frequency components in the images. We demonstrate the effectiveness of our method through thorough quantitative and qualitative analyses on various datasets and models. To the best of our knowledge, this is the first work that addresses the problem of discovering the editing directions in the latent variables of DMs in an unsupervised manner.

% We proposed a method to identify semantic editing directions in the latent space of diffusion models (DMs) using Riemannian geometry. Our method discovers local and global feature directions, revealing the relationship between denoising timestep and the frequency domain that the model focuses on. Additionally, our method demonstrates that the latent space is globally warped and can be applied to stable-diffusion. This work deepens the understanding of DMs and has potential applications in the manipulation and control of these generative models. 

\section{intro}
\paragraph{latent 파자}
% 용현
% Despite the success of DMs as generative models, there has been relatively little research on the latent space within the model. This is due to the fact that the latent space of DMs have no semantic structure. Nevertheless, recent studies \cite{baranchuk2021label,kwon2022diffusion,tumanyan2022plug} have shown that the feature space inside the DMs contain semantic information. It implies that there is a semantic structure corresponding to the latent space.


% As \todo{위 문단의 DM의 latent모름과 GAN의 latent유용을 대조해서 latent 필요성을 대두시키는 문단으로 합치면 좋겠습니다.} shown in Generative Adversarial Networks (GANs) research, understanding the properties and characteristics of this latent space can provide valuable insights into the behavior of generative models and facilitate their analysis and utilization. 
% Further research on this topic has the potential to uncover new ways of utilizing and controlling generative models and improve their performance in various tasks.
In the field of GANs, there have been numerous efforts to analyze the latent space and identify meaningful traversal directions.

% 민기
% Despite the success of DMs as generative models, there has been relatively little research on the feature spaces within the model. This is due in part to the fact that DMs are typically trained on noisy images and output noise, making it difficult to focus on their internal features. 
% However, recent studies including \cite{kwon2022diffusion} have demonstrated the potential of using the feature space within the model. In particular, \citet{kwon2022diffusion} showed that the bottleneck of the U-Net can be used as a semantic latent space and that the space exhibits local linearity.
%\cite{baranchuk2021label,kwon2022diffusion,tumanyan2022plug}
% It is indeed interesting to discover that there exists a linear semantic latent space within the DM that corresponds to inputs close to Gaussian noise.
\paragraph{local vs global}
Sample-wise methods of local latent space manipulation \cite{ramesh2018spectral,patashnik2021styleclip,abdal2021styleflow} have been proposed, as well as global manipulation techniques \cite{harkonen2020ganspace,shen2021closed,yuksel2021latentclr} that operate on the entire latent space. \yh{More recently, several studies \cite{zhu2021low, choi2021not} have been examine the geometrical properties of the latent space in GANs and utilize these findings for image manipulations.}

% More recently, \citet{choi2021not} introduced both local and global manipulation techniques, which we refer to these as the local and global basis, with a focus on the geometry of the latent space in StyleGAN2.


% By taking this geometrical approach to analyzing the latent space of the DMs, we expect to gain new insights into its capabilities and potential for image processing.

% \yh{In DMs research, \citet{kwon2022diffusion}, for the first time, showed that we could discover the meaningful direction in the bottleneck of the U-Net with supervised method. They focused on the existence of editable direction itself, but we pay attention more to the experiment result that these directions have local linear properties. (e.g. enable vector addition) This is because it implies geometric information about the feature space of the DM. We expected that this would allow us to analyze DM's latent space with geometrical approach.}

% previous
% In \todo{Despite~ 문단의 후반부 However~를 이쪽으로 합치면 좋겠습니다.} contrast to these approaches, \citet{kwon2022diffusion} demonstrated the ability to edit directions in the bottleneck of DMs \todo{전개에 중요한 부분인데 한문장으로 휙 넘어가기보다는 한번 끊고 무게를 실어주세요. local linearity도 뒤에 나올거라서 미리 한번 설명해두면 좋겠습니다.} but did not provide a detailed analysis or explanation of the results. 

\paragraph{Riemannian}
% The latent variables of the model are assumed to be approximately Gaussian distributed, allowing them to be treated as a Riemannian space. To better understand the intractable \exspace{}, latent variables, we map it onto the more tractable \ehspace{}, which is the bottleneck and has been experimentally shown to exhibit local linearity.

% previous version
% The aim of this study was to investigate the latent space of a diffusion model using techniques from Riemannian geometry. To accomplish this, we first obtained local bases for the exspace and ehspace by performing singular value decomposition (SVD) on the Jacobian matrix. The homogeneity observed across local directions in the ehspace allowed us to construct a global basis for the purpose of editing various images. 

%%%%%%% method trash bin
% Throughout this paper, we will make use of several concepts from differential geometry.
% (e.g., tangent space or metric)
% In order to make the paper self-contained, we will provide a brief introduction to the key concepts that are used in our work.
% For a more in-depth treatment of these concepts, please refer to the references provided in section \ref{}.
%To make this paper self-contained, we will give a brief introduction to the basic concept we use in this work. Please refer to \ref{} for more detailed descriptions.

% 간단 버전
% Differential geometry is concerned with the study of curved spaces, often referred to as \emph{manifold} $\mathcal{M}$. Differential geometry allows us to attach a local vector space, known as the \emph{tangent space}, at any point in a manifold. The tangent space, denoted as $\tanxspace{}$, can be thought of as the space of all possible velocity vectors of curves traveling through the point $\mathbf{x}$.

% In linear algebra, all geometrical concepts such as norms and angles are defined using an inner product, specifically the dot product. In order to extend these concepts to a curved manifold, we need a corresponding inner product known as the \emph{metric}, denoted as $\metric{}$. The metric can be thought of as the usual inner product $\metric{}_\mathbf{x}$ in a vector space $\tanxspace{}$ when the tangent space is specified. The geometrical structure (e.g. curvature) of the manifold can only be determined by using the metric.

% In the field of differential geometry, when information about the geometric structure of a given space is limited or unavailable, a useful tool for analysis is the concept of the \emph{pullback metric}. The applicability of this metric is determined by the presence of a smooth map between the metric-free space to metric-enabled space. In our context, pullback metric of \ehspace{} is utilized to measure the length of direction on the \exspace{} without prior knowledge of its metric.

% \paragraph{manifold.} 
% Differential geometry is concerned with the study of curved spaces, often referred to as \emph{manifold} $\mathcal{M}$.
%The main object of differential geometry is to manage the curved space. In differential geometry, the curved space usually refers to \emph{manifold} $\mathcal{M}$. 

% Definition of manifold
% The manifold is a space that has a homeomorphism between the local open set to $\mathbb{R}^n$ Euclidean ball. Homeomorphism is a function which is a bijection, and forward and inverse maps are both continuous. 

% \paragraph{tangent space.} 
% Differential geometry allows us to attach a local vector space, known as the \emph{tangent space}, at any point in a manifold. The tangent space, denoted as $\tanxspace{}$, can be thought of as the space of all possible velocity vectors of curves traveling through the point $\mathbf{x}$.
% In differential geometry, one can attach local vector space called \emph{tangent space}, denoted as $\tanxspace{}$, at any point in the manifold. The most intuitive definition of tangent space is to consider all the velocity vectors of curves traveling through the point $\mathbf{x}$.

% \paragraph{metric.} 
% In linear algebra, all geometrical concepts such as norms and angles are defined using an inner product, specifically the dot product. In order to extend these concepts to a curved manifold, we need a corresponding inner product known as the \emph{metric}, denoted as $\metric{}$. This point-wise inner product is defined in the tangent space and can be thought of as the usual inner product $\metric{}_\mathbf{x}$ in a vector space $\tanxspace{}$ when the tangent space is specified.
%We also need the corresponding concept of inner-product for a curved manifold. The \emph{metric}, denoted by $\metric{}$, is point-wise inner-product defined in the tangent space. By specifying the tangent space, we could consider $\metric{}_\mathbf{x}$ as the usual inner product in a vector space $\tanxspace{}$. 

% 새롭게 쓴 부분
% \paragraph{pullback metric.} 
% In the field of differential geometry, when information about the geometric structure of a given space is limited or unavailable, a useful tool for analysis is the concept of the \emph{pullback metric}. The applicability of this metric is contingent upon the presence of a diffeomorphism between the metric-free space (e.g. \exspace{}) to metric-enabled space (e.g. \ehspace{}). In our context, this metric is utilized to measure the length of direction on the \exspace{} without prior knowledge of its metric.

% \subsection{Local Direction}

% Here, we present a method for discovering interpretable directions of the latent variables of a given image in DMs. We leverage the \ehspace{}, which has been shown to possess a semantically meaningful structure, to uncover important directions in the \exspace{}, which lacks such a structure. Specifically, our method seeks directions in \exspace{} that maximize the variation in the feature space, \ehspace{}. We provide a theoretical justification for this approach through the lens of Riemannian geometry, demonstrating that it is the natural way to identify meaningful directions of the latent variable.

%Here, we aim to find semantic directions for a given image. Since the latent space of diffusion models (DM) does not have semantic structure, we rely on \ehspace{} to discover the important direction in \exspace{}. To summarize our method, it is yet another approach for finding directions which maximize the variation in feature space. Nevertheless, we explain why such a method is a natural way to find important directions through the lens of Riemannian geometry.
 
 % Given a pretrained DM $\tepsilont : \mathcal{X} \times T \rightarrow \mathcal{E}$, we can predict noise $\epsilon$ from a pair of an input image $\mathbf{x}$ and timestep $t$. The \ehspace{}, referred to as $\mathcal{H}$, is the deepest feature map in UNet model used by DM.
%Given a pretrained DM $\epsilon_{\theta} : \mathcal{X} \times T \rightarrow \mathcal{E}$, from a pair of an input image and timestep $(\mathbf{x}, t)$ to predicted noise $\epsilon$, let $\mathcal{H}$ called \ehspace{} be the deepest feature map in UNet model. 

% The UNet architecture of the DM allows for the creation of a differentiable map between \exspace{} and \ehspace{}, denoted as $f : \mathcal{X} \times T \rightarrow \mathcal{H}$. 
%By design of UNet architecture, we have a differentiable map between \exspace{} and \ehspace{} $f : \mathcal{X} \times T \rightarrow \mathcal{H}$. 
% If we assume that both $\mathcal{X}$ and $\mathcal{H}$ are differentiable manifolds, differential geometry tells us that this map has a corresponding linear map $\jacx{} : \tanxspace{} \rightarrow \tanhspace{}$, called \emph{jacobian} of $f$ at $\mathbf{x}_t$, where $\mathbf{h}_t = f(\mathbf{x}_t)$.
%If we assume $\mathcal{X}$ and $\mathcal{H}$ are differentiable manifolds, the result from differential geometry gives us linear map $df_{\mathbf{x}} : \tanxspace{} \mathcal{X} \rightarrow \tanhspace{}\mathcal{H}$ called \emph{differential} of $f$ at $\mathbf{x}$, where $\mathbf{h} = f(\mathbf{x})$.
% The matrix representation of $\jacx{}$ is known as the jacobian matrix. 
% The jacobian $\jacx{}$ can be thought of as a function that maps directions in the \exspace{} to directions in the \ehspace{}. To reduce the computational cost, we use an average pooled feature map as \ehspace{}.
%The differential of a map can be understood as a function between the direction of domain and image of given map. To release the computational cost of jacobian matrix, we use an average pooled feature map as \ehspace{}.

% We assume that the metric $\metric{}$ at $\mathbf{h}$ is a dot product (i.e. euclidean metric) to assign the geometrical structure in $\mathcal{H}$. This assumption is based on the fact that the directions in \ehspace{} have a local linear property \cite{kwon2022diffusion}.

%To assign the geometrical structure in $\mathcal{H}$, we assume the metric $\metric{}$ at $\mathbf{h}$ is a dot-product. (i.e. euclidean metric) Here, we leveraged the fact that the direction in \ehspace{} has local linear property. \ref{} 

%In order to assign a geometric structure to \exspace{}, we use the pullback metric, defined as $\metric{}_{\mathbf{x}}$, which is based on the metric $\metric{}_{\mathbf{h}}$ defined at $\mathcal{H}$. Now, we could measure the norm of the tangent vector $\dx{} \in \tanxspace{}$ with the pullback metric $\metric{}_\mathbf{x}$.

%\begin{equation}
%\begin{aligned}
%||\dx{}||^2 \triangleq \langle \dx{}, \dx{} \rangle_{\mathbf{x}} = \langle \dh{}, \dh{} \rangle_{\mathbf{h}} = \dx{}^{\top} \jacx{}^{\top} \jacx{}\dx{}
%\end{aligned}
%\end{equation}

% The pullback metric is given by: 
% \begin{equation}
%  f^* \metric{}_{\mathbf{x}} : (v, w) \mapsto \langle df (v), df (w) \rangle_\mathbf{h} 
%  \\
% \end{equation}
% where $v,w \in \tanxspace{}\mathcal{X}, \mathbf{h} = f(\mathbf{x})$. This metric allows us to measure lengths and angles by passing the direction from a metric-free space to a metric-given space.

%용현쓰가 써둔것
% Using the metric $\metric{}$ defined at $\mathcal{H}$, we can also assign a geometric structure to \exspace{}, with \emph{pullback} metric by $f$. The pullback metric $f^* \metric{}$ is defined as below.
% \begin{equation}
%  f^* \metric{}_{\mathbf{x}} : (v, w) \mapsto \langle df (v), df (w) \rangle_\mathbf{h} 
%  \\
% \end{equation}
% where $v,w \in \tanxspace{}\mathcal{X}, \mathbf{h} = f(\mathbf{x})$. The pullback metric is nothing more than a measure of length or angle by passing the direction from a metric-free space to a metric-given space. 

%%%%%%%%%%%%민기쓰
%By utilizing the pullback metric, we can define a unit vector $v_1 \in \tanxspace{}$ as an interpretable direction. This direction is chosen to have the maximum norm with respect to the pullback metric, and can be found by maximizing $\dx{}^{\top} \jacx{}^{\top} \jacx{}\dx{}$. In practice, this can be done by decomposing $\jacx{} = U S V^{\top}$ and finding its first right singular vector, which gives us the same direction as the first eigenvector of $\jacx{}^{\top} \jacx{} = V S^2 V^{\top}$. 

%To uncover additional interpretable directions, we can repeat the process and find the second unit vector $v_2$ that maximizes the norm while remaining orthogonal to the first direction $v_1$. By constraining $v_2$ to the subspace of tangent space of $\tanxspace{}  \backslash \text{span}(v_1)$, we can obtain the second eigenvector of $\jacx{}^{\top} \jacx{}$. This process can be repeated to uncover k meaningful directions in \exspace{}.
%With this method, we are able to extract a meaningful and interpretable direction from the \exspace{}, providing us with a tool for analyzing and manipulating the diffusion model. 

%These directions allow us to understand the behavior and structure of the model in a more intuitive and comprehensive way, and can be used to effectively edit and control the output of the model. In \sref{}, we will demonstrate the effectiveness of this approach through various experimental results and provide analysis.

%% 용현쓰
% As an interpretable direction, we choose unit vector $v_1 \in \tanxspace{}\mathcal{X}$ that has a maximum norm with respect to the pullback metric $f^* \metric{}$. To maximize $v^{\top} J(\mathbf{x})^{\top} J(\mathbf{x}) v$, we could easily find that the $v_1$ is the the first eigenvector of $\jacx{}(\mathbf{x})^{\top} J(\mathbf{x})$. In other word, $v_1$ is the first right singular vector of $\jacx{}(\mathbf{x})^{\top} J(\mathbf{x})$. In practice, we just decompose $\jacx{}(\mathbf{x})$ to find $v_1$, since its right singular vector gives us the same direction.

% Moreover, we could find another direction $v_2$ by finding the second unit vector such that maximizes the norm while orthogonal to the first direction $v_1$. 
% The only change here is to constrain $v_2$ in the subspace of tangent space $\tanxspace{}\mathcal{X}  \backslash \text{span}(v_1)$. Following the same process, we get the second direction $v_2$, which is the second eigenvector of $ J(\mathbf{x})^{\top}  J(\mathbf{x})$. Repetition of the same process can uncover k meaningful directions in \exspace{}.

%%%%%%%%%%%% 민기쓰
%Given a linear map $\jacx{}$ between $\tanxspace{}$ and $\tanhspace{}$, we can also find interpretable directions in the \ehspace{}, denoted as $\dh{}_k \in \tanhspace{}$, by converting directions in the \exspace{}, denoted as $\dx{}_k \in \tanxspace{}$. In Section \ref{}, we will demonstrate that the \ehspace{} direction is more useful for constructing a global basis due to the flatness of the manifold in \ehspace{}. To convert $\dx{}_k$ to $\dh{}_k$, we multiply the inverse of k-th singular value $\sigma_k$ to preserve the euclidean norm of $\dh{}_k$ as 1. This is expressed as:
%\begin{align}
%    \dh{}_k = \sigma_k^{-1}  \jacx{} \dx{}_k
%\end{align}
%Based on the manifold hypothesis, we posit that the image manifold in the \ehspace{} is a lower-dimensional manifold embedded in $\mathcal{H}$. Therefore, by selecting k directions and spanning them, we can treat it as a low-rank approximation of the tangent space. From now on, when we say tangent space, we mean a k-dimensional approximation of the original tangent space. \todo{eigenvalue cdf 의 상위 50 을 dynamic 하게 k 로 사용했다는 것}. The interpretable directions that we find become the local basis of this tangent space.

% Throughout this paper, we will denote a low-dimensional approximation of tangent space as $\tanhspace{}\mathcal{\Tilde{H}}$, and call their basis a \emph{local basis} at $\mathbf{h}$.

%In summary, we have shown that the right singular vectors of $\jacx{}$ correspond to interpretable directions in the \exspace{}, while left singular vectors correspond to the corresponding directions in the \ehspace{}. Moreover, we construct low dimenstional approximation of the tangent space $\tanxspace{}$ and $\tanhspace{}$ by spanning the k local directions discovered.

% 용현쓰
% Since we have linear map $df$ between $\tanxspace{}\mathcal{X}$ to $\tanhspace{}\mathcal{H}$, we could find interpretable direction in \ehspace{} $\dh{}_k \in \tanhspace{}\mathcal{H}$ by converting the direction in \exspace{} $\dx{}_k \in \tanxspace{}\mathcal{X}$. When converting $\dx{}_k$ to $\dh{}_k$, we multiply the inverse of the singular value $\sigma_i$ to maintain $\dh{}_k$ as a unit vector.

% \begin{align}
%     \dh{}_k = \sigma_k^{-1}  J(\mathbf{x}) \dx{}_k
% \end{align}

% % 작성중.. direction 으로 basis 만들기
% Following the manifold hypothesis, we postulate the image manifold in \ehspace{} is a lower-dimensional manifold embedded in $\mathcal{H}$. Thus, we select k direction and span them to consider it as a low-rank approximation of tangent space. 

% In conclusion, we found that right singular vectors of $\jacx{}(\mathbf{x})$ refers to local interpretable direction in \exspace{}, while left singular vectors is refers to the corresponding direction in the \ehspace{}. 

%\subsection{Geodesic Shooting}
